Large Multiuser MIMO Detection: Algorithms and Architectures

In this thesis, we investigate the problem of efficient data detection in large MIMO and high order MU-MIMO systems. First, near-optimal low-complexity detection algorithms are proposed for regular MIMO systems. Then, a family of low-complexity hard-output and soft-output detection schemes based on channel matrix puncturing targeted for large MIMO systems is proposed. The performance of these schemes is characterized and analyzed mathematically, and bounds on capacity, diversity gain, and probability of bit error are derived. After that, efficient high order MU-MIMO detectors are proposed, based on joint modulation classification and subspace detection, where the modulation type of the interferer is estimated, while multiple decoupled streams are individually detected. Hardware architectures are designed for the proposed algorithms, and the promised gains are verified via simulations. Finally, we map the studied search-based detection schemes to low-resolution precoding at the transmitter side in massive MIMO and report the performance-complexity tradeoffs.

==> ack.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Acknowledgments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter*{Acknowledgements}
\addcontentsline{toc}{chapter}{Acknowledgements}
\hspace{1.5cm}

First, I would like to thank my advisor, Prof. Mohammad Mansour and my co-advisor, Prof. Ali Chehab, for their continuous moral and technical support over the past five years. They had given me the opportunity to pursue my Ph.D. on an interesting research topic in a very stimulating research environment. My very special thanks also go to Prof. Ayman Kayssi, who alongside Prof. Ali Chehab believed in my potentials and admitted me to an accelerated Ph.D. program.

I would like to express my sincere appreciation to my dissertation committee members, Dr. Louay Jalloul, Prof. Louay Bazzi, and Prof. Francisco Monteiro. In fact, the impact that the committee members had on me goes far beyond their constructive feedback on my dissertation. Dr. Jalloul had given me a window towards the work in industry through fruitful discussions at an early stage in my research work, Prof. Bazzi has taught me two of the most interesting graduate courses, and Prof. Monteiro was so generous to refer me to relevant research in the community during the first conference that I attended.

I am grateful to many more professors who taught me graduate courses at AUB. In particular, I would like to thank Prof. Zaher Dawy, Prof. Ibrahim Abou Fayssal, Prof. Youssef Nasser, and Prof. Imad Elhajj for making me a more proficient person. Furthermore, I would like to thank the staff at the Maroun Semaan Faculty of Engineering and Architecture, in particular Ms. Rabab Abi Shakra, who helped me in all the logistic details throughout my years at AUB. %, and Mr. Ali Kaafarani and Mr. Saad Itani who have supported me with all the necessary software programs and computational resources.

I would also like to extend my gratitude to the National Council for Scientific Research for partially financing my research.

To Ashraf, Iyad, Jamal, Oussama, Raghid, Saleem, Wissam, and Yamen, thank you for listening, offering me advice, and supporting me through this entire process. You all are the best friends anyone could ever ask for.

Words fail me to express my appreciation to my parents, Akram and Sania, for their love and support, and to my sister's family, Naja, Inas, and Yamen, for the emotional support, and caring.

